Tuning Trains Speed in Railway Scheduling

Railway scheduling consists in ensuring that a set of trains evolve in a shared rail network without collisions, while meeting schedule constraints. This problem is notoriously difficult, even more in the case of uncertain or even unknown train speeds. We propose here a modeling and verification approach for railway scheduling in the presence of uncertain speeds, encoded here as uncertain segment durations. We formalize the system and propose a formal translation to parametric timed automata. As a proof of concept, we apply our approach to benchmarks, for which we synthesize using IMITATOR suitable valuations for the segment durations.

==> tikzlibrarytrambws.code.tex <==
\ProvidesFile{tikzlibrarytrambws.code.tex}
\usetikzlibrary{backgrounds}
\colorlet{lliwytram}{red!75!black}
\colorlet{lliwffenestri}{gray!75!blue}
\colorlet{lliwolwynion}{gray!75}
\tikzset{
  lliw y tram/.code={
        \colorlet{lliwytram}{#1}
  },
  lliw ffenestri/.code={
        \colorlet{lliwffenestri}{#1}
  },
  lliw olwynion/.code={
        \colorlet{lliwolwynion}{#1}
  },
  olwyn/.style={circle, draw, line width=#1*.8pt, minimum width=#1*5pt, inner sep=0pt, fill=lliwolwynion},
  pics/tram/.style={
        code={
          \path [draw, line width=#1*.8pt]
          coordinate (tram) ++(-.2*#1,#1*2.75pt) node (w1) [olwyn=#1] {}
                  ++(#1*.425,0) node (w2) [olwyn=#1] {}
                  ++(#1*.425,0) node (w3) [olwyn=#1] {};
          \path [draw, fill, line width=#1*.4pt]
                (w1) circle (#1*1pt)
                (w2) circle (#1*1pt)
                (w3) circle (#1*1pt);
          \path [draw, left color=lliwytram, right color=lliwytram!20, line width=#1*.4pt]
                (tram) ++(-.4*#1,#1*1.5pt) coordinate (t1) |- ++(#1*1.25,#1*.35) coordinate (t2) |- (w3.south east -| w3.east) |- (w3.west) |- (w2.south east -| w2.east) |- (w2.west) |- (w1.south east -| w1.east) |- (w1.west) -- (w1.south west -| w1.west) -| cycle
                (t1 -| t2) ++(-.05*#1pt,#1*4pt) coordinate (t3) |- ++(-.175*#1,#1*.175) coordinate (t4) |- cycle
                (t3 -| t4) ++(-.5*#1pt,0) |- ++(-.25*#1,.175*#1) coordinate (t5) |- cycle
                (t3 -| t5) ++(-.5*#1pt,0) |- ++(-.25*#1,.175*#1) coordinate (t6) |- cycle
                (t3 -| t6) ++(-.5*#1pt,0) |- ++(-.25*#1,.175*#1) coordinate (t7) |- cycle
                (t3 -| t7) ++(-.5*#1pt,0) |- ++(-.25*#1,.175*#1) coordinate (t8) |- cycle;
          \scoped [on background layer] \fill [left color=lliwffenestri!50, right color=lliwffenestri!10] (t3) rectangle (t8);
        }
  }
}
\endinput

